Damped energy-norm a posteriori error estimates for fully discrete approximations of the wave equation using C2-reconstructions with the leapfrog scheme

We derive a posteriori error estimates for the the scalar wave equation discretized in space by continuous finite elements and in time by the explicit leapfrog scheme. Our analysis combines the idea of invoking extra time-regularity for the right-hand side, as previously introduced in the space semi-discrete setting, with a novel, piecewise quartic, globally twice-differentiable time-reconstruction of the fully discrete solution. Our main results show that the proposed estimator is reliable and efficient in a damped energy norm. These properties are illustrated in a series of numerical examples.

==> figures/propagating/solution/solution.tex <==
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$x$},
	ylabel={},
	width=\textwidth,
	xmin=-10,
	xmax= 10,
	ymin=- 1,
	ymax=  1
]

\plot[solid,thick] table[x=x,y=u] {figures/propagating/solution/data/snapshot_04.txt};

\end{axis}
\end{tikzpicture}
\subcaption{$t=4$}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$x$},
	ylabel={},
	width=\textwidth,
	xmin=-10,
	xmax= 10,
	ymin=- 1,
	ymax=  1
]

\plot[solid,thick] table[x=x,y=u] {figures/propagating/solution/data/snapshot_05.txt};

\end{axis}
\end{tikzpicture}
\subcaption{$t=5$}
\end{minipage}

\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$x$},
	ylabel={},
	width=\textwidth,
	xmin=-10,
	xmax= 10,
	ymin=- 1,
	ymax=  1
]

\plot[solid,thick] table[x=x,y=u] {figures/propagating/solution/data/snapshot_08.txt};

\end{axis}
\end{tikzpicture}
\subcaption{$t=8$}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$x$},
	ylabel={},
	width=\textwidth,
	xmin=-10,
	xmax= 10,
	ymin=- 1,
	ymax=  1
]

\plot[solid,thick] table[x=x,y=u] {figures/propagating/solution/data/snapshot_12.txt};

\end{axis}
\end{tikzpicture}
\subcaption{$t=12$}
\end{minipage}

\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$x$},
	ylabel={},
	width=\textwidth,
	xmin=-10,
	xmax= 10,
	ymin=- 1,
	ymax=  1
]

\plot[solid,thick] table[x=x,y=u] {figures/propagating/solution/data/snapshot_15.txt};

\end{axis}
\end{tikzpicture}
\subcaption{$t=15$}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$x$},
	ylabel={},
	width=\textwidth,
	xmin=-10,
	xmax= 10,
	ymin=- 1,
	ymax=  1
]

\plot[solid,thick] table[x=x,y=u] {figures/propagating/solution/data/snapshot_20.txt};

\end{axis}
\end{tikzpicture}
\subcaption{$t=20$}
\end{minipage}



==> figures/standing/solution/solution.tex <==
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$t$},
	ylabel={}, %ylabel={$2(t-t_0)e^{-(t-t_0)^2}$},
	width=\textwidth,
	xmin= 0,
	xmax=10
]

\plot[solid,thick] table[x=t,y=f] {figures/standing/solution/data/profile.txt};

\end{axis}
\end{tikzpicture}
\subcaption{right-hand side}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$t$},
	ylabel={}, %ylabel={$\psi(t)$},
	width=\textwidth,
	xmin= 0,
	xmax=10
]

\plot[solid,thick] table[x=t,y=u] {figures/standing/solution/data/profile.txt};

\end{axis}
\end{tikzpicture}
\subcaption{solution}
\end{minipage}


==> figures/standing_m10/solution/solution.tex <==
\begin{figure}
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$t$},
	ylabel={$2(t-t_0)e^{-(t-t_0)^2}$},
	width=\textwidth,
	xmin= 0,
	xmax=10
]

\plot[solid,thick] table[x=t,y=f] {figures/standing/solution/data/profile.txt};

\end{axis}
\end{tikzpicture}
\subcaption{right-hand side}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}
\begin{axis}
[
	xlabel={$t$},
	ylabel={$\psi(t)$},
	width=\textwidth,
	xmin= 0,
	xmax=10
]

\plot[solid,thick] table[x=t,y=u] {figures/standing/solution/data/profile.txt};

\end{axis}
\end{tikzpicture}
\subcaption{solution}
\end{minipage}

\caption{Time profiles in the standing wave example}
\end{figure}


==> numerics.tex <==
\subsection{Setting}

In these examples, we consider the one-dimensional domain $\Omega := (-L,L)$ with $L := 10$,
and set the computational time to $T_\star := 1000$. For the values of $\rho$ employed hereafter,
this final time is such that $e^{-\rho T_\star} \leq 5 \cdot 10^{-6}$ in all simulations, so that
stopping the simulation has little effect. We use uniform meshes, and finite elements of degree
$1 \leq p \leq 3$. We emloy mesh sizes ranging from $h=10$ to, $0.039$, meaning that the interval
$\Omega$ is divided into at least $2$ and at most $512$ elements.

For each $p$, we denote by $\alpha_p$ the largest value for which the leap-frog scheme
is stable with $\tau = \alpha_p h$.  We emprically found these values to be $\alpha_1 = 0.59$,
$\alpha_2 = 0.26$ and $\alpha_3 = 0.15$. In our examples, given $h$, we fix the time step by setting
$\tau = r\alpha h$, with $r \in (0,1)$. Unless explicitely specified, we use $r=0.9$.

When $p=3$, we also employ finer time-step values so that the order of the time-discretization
error matches the one of the space discretization. To do so, we fix $\tau_0 = r_0 \alpha_3 h_0$
for the coarsest computational mesh where $h = h_0 = 10$, and then adjust $\tau$ so that
$\tau^3/h^2$ remains constant for all meshes. This is indicated by the notation ``$\tau^3 \sim h^2$''
in the graphs below.

We use two different analytical solutions for these bencharmarks, respectively
corresponding to ``standing'' and ``propagating'' waves. For the standing wave,
we set
\begin{equation*}
f(t,x) := -2(t-t_0)e^{-(t-t_0)^2}\sin(a(x-L))
\end{equation*}
where $t_0 := 4$ and $a = m\pi/(2L)$ with $m = 5$. Notice that although $f$ does
exactly not vanish at $t=0$, we do have
$|f(0,\cdot)| \leq 8 e^{-16} \leq 0.9 \cdot 10^{-6}$,
$|\dot f(t,\cdot)| \leq 62 e^{-16} \leq 7.0 10^{-6}$
and
$|\ddot f(t,\cdot)| \leq 464 e^{-16} \leq 5.3 \cdot 10^{-5}$, whereas
$\max_{t,x} |f(t,x)| \geq 0.5$. The corresponding solution reads
\begin{equation*}
u(t,x)
=
\Re \psi(t-t_0)
\sin(a(x-L))
\end{equation*}
with
\begin{equation*}
\psi(t)
:=
\int_{-\infty}^{t} e^{-\theta^2-ia \theta} d\theta e^{ia t}.
\end{equation*}
To see that, observe that
\begin{equation*}
\ddot \psi(t) = (-2t+ia)e^{-t^2} - a^2\psi(t),
\end{equation*}
so that
\begin{equation*}
\Re (\ddot \psi+a^2\psi) = -2te^{-t^2}.
\end{equation*}
We observe again that $|u(0,\cdot)| \leq 1.1 \cdot 10^{-8}$
and $|\dot u(0,\cdot)| \leq 8.3 \cdot 10^{-8}$ whereas
$\max_{t,x} |u(t,x) \geq 4 \cdot 10^{-2}$, so that setting the initial
conditions to zero incures an error much smaller than the discretization error.
The time profile of $f$ and $u$ are represented on Figure \ref{figure_solution_standing}.
In practice, we compute $\psi$ with the {\tt erf} function of {\tt Faddeeva} software
package by observing that
\begin{equation*}
\psi(t)
=
e^{-a^2/4+iat} \int_{-\infty}^t e^{-(\theta+ia/2)^2} d\theta
=
e^{-a^2/4+iat} \int_{-\infty}^{t+ia/2} e^{-z^2} dz.
\end{equation*}

For the example with the propagating wave, we set
\begin{equation*}
f(t,x)
:=
-2(t-t_0)e^{-(t-t_0)^2} e^{-x^2}
\end{equation*}
where, again $t_0 := 4$. The solution in full space reads
\begin{equation*}
u_\infty(t,x)
:=
\frac{1}{4}
\left (
e^{(t-t_0+x)^2/2} \int_{-\infty}^{t-t_0+x} e^{-\tau^2/2} d\tau
+
e^{(t-t_0-x)^2/2} \int_{-\infty}^{t-t_0-x} e^{-\tau^2/2} d\tau
\right )
e^{-(x^2+(t-t_0)^2)}.
\end{equation*}
This expression is obtained by simplifying the representation
\begin{equation*}
u_\infty(t,x)
=
\frac{1}{2}
\int_{y=-\infty}^{+\infty} \int_{\theta > |y|} f(t-\theta,x-y) d\theta dy
\end{equation*}
stemming from the Green's function $\mathbf 1_{t > |x|}$
of the one-dimensional wave equation in free-space.
Notice that $u_\infty$ does not satisfy the Dirichlet boundary conditions
at $x = \pm L$. However, we can obtain the correct solution by using
the mirror image principle, and setting
\begin{equation*}
u(t,x) = u_\infty(t,x) + \sum_{n=1}^{+\infty} (-1)^n \left (
u_\infty(t, 2nL+(-1)^n x)
+
u_\infty(t,-2nL+(-1)^n x)
\right ).
\end{equation*}
One readily checks that $u$ satisfies the boundary conditions on $x \pm L$.
As above, we do not have $u(0,\cdot) = 0$, but the initial values are small
enough that they do not affect the numerical experiments. Notice that $u$
in fact solves the wave equation over $\mathbb R \times \mathbb R$ with
right-hand side
\begin{equation*}
\widetilde f(t,x) = f(t,x) + \sum_{n=1}^{+\infty} (-1)^n \left (
f(t, 2nL+(-1)^n x)
+
f(t,-2nL+(-1)^n x)
\right ),
\end{equation*}
but the different $\widetilde f - f$ is small enough over $\Omega$ that it does
not interfere with our experiments. Finally, for any finite time $t \geq 0$ and
$x \in \Omega$, the terms in the series defining $u(t,x)$ decay superalgebraically.
For our simulations, we simply compute the sum over $1 \leq n \leq 50$. As above,
we use the {\tt Faddeva} software package to evaluate the integral of the Gaussian
numerically.

\input{figures/standing/solution/solution}

\input{figures/propagating/solution/solution}

\subsubsection{Error measure}

For ease of read of the graph, we introduce shot-hand notation for the errors.
Specifically, we compare
\begin{equation*}
e^2(u) := \int_0^{+\infty} \|u(t)-u_{h\tau}(t)\|_\Omega^2 e^{-2\rho t} dt,
\qquad
e^2(w) := \int_0^{+\infty} \|u(t)-w_{h\tau}(t)\|_\Omega^2 e^{-2\rho t} dt
\end{equation*}
with
\begin{equation*}
e^2(\sfU) := \tau \sum_{n = 0}^{+\infty} \|u(t_n)-\sfU^n\|_\Omega^2 e^{-2\rho t_n}
\end{equation*}
on Figure \ref{figure_reconstruction} and
\begin{equation*}
e_x^2(u) := \int_0^{+\infty} \|\nabla(u(t)-u_{h\tau}(t))\|_\Omega^2 e^{-2\rho t} dt,
\qquad
e_x^2(w) := \int_0^{+\infty} \|\nabla(u(t)-w_{h\tau}(t))\|_\Omega^2 e^{-2\rho t} dt
\end{equation*}
with
\begin{equation*}
e_x^2(\sfU) := \tau \sum_{n = 0}^{+\infty} \|\nabla(u(t_n)-\sfU^n)\|_\Omega^2 e^{-2\rho t_n}
\end{equation*}
on Figure \ref{figure_reconstruction_space}. Finally, Figure \ref{figure_reconstruction_time}
compares
\begin{equation*}
e_t^2(u) := \int_0^{+\infty} \|\dot u(t)-\dot u_{h\tau}(t)\|_\Omega^2 e^{-2\rho t} dt,
\qquad
e_t^2(w) := \int_0^{+\infty} \|\dot u(t)-\dot w_{h\tau}(t)\|_\Omega^2 e^{-2\rho t} dt
\end{equation*}
and
\begin{equation*}
e_t^2(\sfU) := \tau \sum_{n = 0}^{+\infty} \|\dot u(t_n)-\tau^{-1}(\sfU^{n+1}-\sfU^{n-1})\|_\Omega^2 e^{-2\rho t_n}.
\end{equation*}
Besides, we also set $\xi^2 = e_t^2(w)+e_x^2(w)$.

In practice, these integrals and sums are computed up to $t=T_\star$. As argued above,
$T_\star$ as been chosen in such a way that the tail of the integrals and series is negligeable.

\subsubsection{Estimator}

To estimate the error, we construct a continuous piecewise polynomial function $\sigma_{h\tau}$
such that
\begin{equation*}
\partial_x \sigma_{h\tau} = f_\tau-\ddot w_{h\tau}.
\end{equation*}
A simple integration by parts then reveals that
\begin{equation*}
\|\calR(t)\|_{V'}^2
\leq
\|\partial_x w_{h\tau}(t)+\sigma_{h\tau}(t)\|_\Omega.
\end{equation*}
As a result, introducing
\begin{equation*}
R^2
:=
\int_0^{+\infty} \|\partial_x w_{h\tau}(t)+\sigma_{h\tau}(t)\|_\Omega e^{-2\rho t} dt.
\end{equation*}
and
\begin{equation*}
M^2
:=
\frac{1}{\rho^2} \int_0^{+\infty} \|\partial_x (\dot u_{h\tau}(t) - \dot w_{h\tau}(t))\|_\Omega^2 e^{-2\rho t} dt,
\end{equation*}
the estimate in \eqref{eq:error_upper_bnd} ensures that
\begin{equation*}
\xi \leq \eta + \operatorname{h.o.t.}
\end{equation*}
with
\begin{equation*}
\eta^2 = R^2 + 10 M^2.
\end{equation*}

\subsection{Accuracy of the reconstructions}

The goal of this first example is to highlight that the reconstructions
$u_{h\tau}$ and $w_{h\tau}$ obtained from the time-step values $\sfU$
have the expected accuracy.

For simplicity, we focus on the standing wave example with $\rho = 0.02$.
We obtained very similar results in the with different values of $\rho$
and in the propagating wave example. For the sake of shortness, we do not
reproduce all the curves here.

As can be seen of Figures \ref{figure_reconstruction}, \ref{figure_reconstruction_space}
and \ref{figure_reconstruction_time}, all the errors are very close,
as anticipated. We also observe the expected convergence rates.
%%%   no longer relevant with the change of parameter $m=5$.
%%%
%%%   with the exception
%%%   of the $e_x(\cdot)$ and $e_t(\cdot)$ for $p=1$. In this case, however, the apparent
%%%   superconvergence (quadratic instead of linear) is simply a pre-asymptotic effect due
%%%   to the fact that most of the error is due to dispersion (rather than approximation
%%%   properties) for this range of mesh sizes and this value of $\rho$. This is especially
%%%   visible on Figure \ref{figure_reconstruction_time} where the last data point on the
%%%   curve indicates that the convergence is about to slow down. We will also see a similar effect
%%%   when commenting on the accuracy of the estimator later on.

\begin{figure}
\begin{plotpagetitle}{}{$p=1$}
\ploteUv{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e(\sfU)$};
\ploteuv{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e(u)$};
\plotewv{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e(w)$};
\SlopeTriangle{0.7}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}
\begin{plotpagetitle}{}{$p=2$}
\ploteUv{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e(\sfU)$};
\ploteuv{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e(u)$};
\plotewv{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e(w)$};
\SlopeTriangle{0.6}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}

\begin{plotpagetitle}{}{$p=3$}
\ploteUv{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e(\sfU)$};
\ploteuv{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e(u)$};
\plotewv{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e(w)$};
\SlopeTriangle{0.5}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}
\begin{plotpagetitle}{}{$p=3$, $\tau^3 \sim h^2$}
\ploteUv{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e(\sfU)$};
\ploteuv{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e(u)$};
\plotewv{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e(w)$};
\SlopeTriangle{0.5}{-0.1}{0.15}{-3}{$h^3$}{}
\end{plotpagetitle}
\caption{Reconstruction errors}
\label{figure_reconstruction}
\end{figure}

\begin{figure}
\begin{plotpagetitle}{}{$p=1$}
\ploteUx{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_x(\sfU)$};
\ploteux{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_x(u)$};
\plotewx{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_x(w)$};
\SlopeTriangle{0.725}{-0.1}{0.15}{-1}{$h^1$}{}
\end{plotpagetitle}
\begin{plotpagetitle}{}{$p=2$}
\ploteUx{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_x(\sfU)$};
\ploteux{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_x(u)$};
\plotewx{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_x(w)$};
\SlopeTriangle{0.6}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}

\begin{plotpagetitle}{}{$p=3$}
\ploteUx{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_x(\sfU)$};
\ploteux{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_x(u)$};
\plotewx{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_x(w)$};
\SlopeTriangle{0.5}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}
\begin{plotpagetitle}{}{$p=3$, $\tau^3 \sim h^2$}
\ploteUx{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_x(\sfU)$};
\ploteux{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_x(u)$};
\plotewx{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_x(w)$};
\SlopeTriangle{0.5}{-0.1}{0.15}{-3}{$h^3$}{}
\end{plotpagetitle}
\caption{Reconstruction errors on the space deriative}
\label{figure_reconstruction_space}
\end{figure}

\begin{figure}
\begin{plotpagetitle}{}{$p=1$}
\ploteUt{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_t(\sfU)$};
\ploteut{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_t(u)$};
\plotewt{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_t(w)$};
\SlopeTriangle{0.7}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}
\begin{plotpagetitle}{}{$p=2$}
\ploteUt{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_t(\sfU)$};
\ploteut{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_t(u)$};
\plotewt{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_t(w)$};
\SlopeTriangle{0.6}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}

\begin{plotpagetitle}{}{$p=3$}
\ploteUt{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_t(\sfU)$};
\ploteut{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_t(u)$};
\plotewt{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_t(w)$};
\SlopeTriangle{0.5}{-0.1}{0.15}{-2}{$h^2$}{}
\end{plotpagetitle}
\begin{plotpagetitle}{}{$p=3$, $\tau^3 \sim h^2$}
\ploteUt{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.2}{0.5cm}{-90}{$e_t(\sfU)$};
\ploteut{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.4}{0.5cm}{-90}{$e_t(u)$};
\plotewt{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.5}{0.5cm}{ 45}{$e_t(w)$};
\SlopeTriangle{0.5}{-0.1}{0.15}{-3}{$h^3$}{}
\end{plotpagetitle}
\caption{Reconstruction errors on the time deriative}
\label{figure_reconstruction_time}
\end{figure}

\subsection{Standing wave example}

We now focus on the properties of the error estimator,
and we start here in the standing wave example.

\subsubsection{Short-time error control}

We start by setting $\rho = 1$. The corresponding result appear on Figure
\ref{figure_standing_short}, and the following comments are in order.
The ``oscillation'' term $\eta_f$ always superconverges. Besieds,
asymptotically, we indeed obtained a guaranteed bound, and the effictivity
index is at most 3 in all cases. Besides, $p=1$, the estimator seems asymptotically
exact. Since the leap-frog scheme provides a time-discretization error in $\tau^2 \sim h^2$
it is to be expected, as it is in agreement with results observed for the
semi-discrete in \cite{Theo:22}. Similarly, we see in this case that $M$ super-converges.

\begin{figure}
{
\begin{plotpage}
{
	ymax=0,
	ymin=1.e-8
}
\plotR{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.05}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.05}{0.5cm}{-90}{$M$};
\plotF{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.7}{0.5cm}{-90}{$\eta_f$};
\plotE{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.6}{0.5cm}{45}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin = 0.005,
	ymax = 4.000
}
\plotMRE{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.4}{1cm}{0}{$\eta/\xi$};
\plotRE{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.3}{1cm}{-10}{$R/\xi$};
\plotME{figures/standing/data/rho1.00_p0_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-70}{$M/\xi$};
\end{plotpage}
\subcaption{$p=1$}

\begin{plotpage}
{
	ymax=0,
	ymin=1.e-8
}
\plotR{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.05}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.05}{0.5cm}{-90}{$M$};
\plotF{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\plotE{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.6}{0.5cm}{45}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin = 0.005,
	ymax = 4.000
}
\plotMRE{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.4}{1.5cm}{-70}{$\eta/\xi$};
\plotRE{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.8}{1cm}{-90}{$R/\xi$};
\plotME{figures/standing/data/rho1.00_p1_r0.9/data.txt} \plotpin{0.1}{0.5cm}{-70}{$M/\xi$};
\end{plotpage}
\subcaption{$p=2$}

\begin{plotpage}
{
	ymax=0,
	ymin=1.e-8
}
\plotR{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.05}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.05}{0.5cm}{-90}{$M$};
\plotF{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.7}{0.5cm}{-90}{$\eta_f$};
\plotE{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{45}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin = 0.005,
	ymax = 4.000
}
\plotRE{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.95}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.2}{0.5cm}{0}{$M/\xi$};
\plotMRE{figures/standing/data/rho1.00_p2_r0.9/data.txt} \plotpin{0.6}{2.0cm}{-70}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=3$}

\begin{plotpage}
{
	ymax=0,
	ymin=1.e-8
}
\plotR{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.05}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.05}{0.5cm}{-90}{$M$};
\plotF{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.7}{0.5cm}{-90}{$\eta_f$};
\plotE{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.6}{0.5cm}{45}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin = 0.005,
	ymax = 4.000
}
\plotRE{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.95}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.2}{0.5cm}{-45}{$M/\xi$};
\plotMRE{figures/standing/data/rho1.00_p2_sts/data.txt} \plotpin{0.4}{0.5cm}{20}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=3$, $\tau^3 \sim h^2$}
}

\caption{Standing wave example with $\rho=1$}
\label{figure_standing_short}
\end{figure}

\subsubsection{Long-time error control}

We then set $\rho = 0.02$. We still observe a super-convergence of $\eta_f$ for
all values of $p$. Asymptotically, the bound given by $\eta$ is indeed guaranteed,
and the effecitvity index is about 10 at worst in all caes.
For $p=1$, we see that $M$ is in fact the dominant part of the estimator, meaning
that asymptotic regime where the time discretization error should be negligeable
has not been reached yet. This in agreement with the above observation regarding
the convergence rates.

Interestingly, the cases where $p \geq 2$ show that the $M$ component of the
estimator is indeed required to obtain a guaranteed bound. Indeed, in those cases,
$R/\xi \ll 1$, even asymptotically. The question of whether the factor $\sqrt{10}$
in the bound is sharp remains open.

\begin{figure}
{
\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.2}{1cm}{10}{$\xi$};
\plotR{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.65}{0.5cm}{-45}{$R$};
\plotM{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.3}{0.5cm}{180}{$M$};
\plotF{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.01,
	ymax = 100.00
}
\plotMRE{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.5}{0.5cm}{0}{$\eta/\xi$};
\plotRE{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-70}{$R/\xi$};
\plotME{figures/standing/data/rho0.02_p0_r0.9/data.txt} \plotpin{0.35}{0.5cm}{-70}{$M/\xi$};
\end{plotpage}
\subcaption{$p=1$}

\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\plotR{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.55}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.3}{0.5cm}{0}{$M$};
\plotF{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.01,
	ymax = 100.00
}
\plotMRE{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.5}{0.4cm}{ 20}{$\eta/\xi$};
\plotRE{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.8}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/standing/data/rho0.02_p1_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-70}{$M/\xi$};
\end{plotpage}
\subcaption{$p=2$}

\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\plotR{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.70}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.4}{0.5cm}{  0}{$M$};
\plotF{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.01,
	ymax = 100.00
}
\plotMRE{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{ 10}{$\eta/\xi$};
\plotRE{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.95}{0.5cm}{ 90}{$R/\xi$};
\plotME{figures/standing/data/rho0.02_p2_r0.9/data.txt} \plotpin{0.2}{0.5cm}{0}{$M/\xi$};
\end{plotpage}
\subcaption{$p=3$}

\begin{plotpage}
{
	ymin = 1.e-7,
	ymax = 1.e+3
}
\plotE{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\plotR{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.70}{1cm}{-45}{$R$};
\plotM{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.4}{0.5cm}{  0}{$M$};
\plotF{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.01,
	ymax = 100.00
}
\plotRE {figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.70}{0.5cm}{-90}{$R/\xi$};
\plotME {figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.95}{1.5cm}{-90}{$M/\xi$};
\plotMRE{figures/standing/data/rho0.02_p2_sts/data.txt} \plotpin{0.40}{0.5cm}{  0}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=3$, $\tau^3 \sim h^2$}
}

\caption{Standing wave example with $\rho=0.02$}
\label{figure_standing_long}
\end{figure}

\subsection{Propagating wave example}

We continue with the propagating wave example.

\subsubsection{Short-time error control}

We start by setting $\rho=0.20$. Asymptotically, we obtain guaranteed error bounds
with effectitivity indices of $10$ at worst.

\begin{figure}
{
\begin{plotpage}
{
	ymin = 1.e-7,
	ymax = 10
}
\plotR{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.5}{1.0cm}{-135}{$R$};
\plotM{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.15}{0.5cm}{0}{$M$};
\plotF{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\plotE{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.55}{0.5cm}{10}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin =  0.02,
	ymax = 20.00
}
\plotRE{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.8}{0.5cm}{-110}{$M/\xi$};
\plotMRE{figures/propagating/data/rho0.20_p0_r0.9/data.txt} \plotpin{0.4}{0.5cm}{10}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=1$}

\begin{plotpage}
{
	ymin = 1.e-7,
	ymax = 10
}
\plotR{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.55}{1cm}{-45}{$R$};
\plotM{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.3}{0.5cm}{0}{$M$};
\plotF{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\plotE{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 20.00
}
\plotRE{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.8}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.4}{1.5cm}{-90}{$M/\xi$};
\plotMRE{figures/propagating/data/rho0.20_p1_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 20}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=2$}

\begin{plotpage}
{
	ymin = 1.e-7,
	ymax = 10
}
\plotR{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.70}{1cm}{-45}{$R$};
\plotM{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.4}{0.5cm}{  0}{$M$};
\plotF{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\plotE{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 20.00
}
\plotRE{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-45}{$M/\xi$};
\plotMRE{figures/propagating/data/rho0.20_p2_r0.9/data.txt} \plotpin{0.9}{0.5cm}{-45}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=3$}

\begin{plotpage}
{
	ymin = 1.e-7,
	ymax = 10
}
\plotR{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.10}{1.0cm}{-110}{$R$};
\plotM{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.00}{0.5cm}{   0}{$M$};
\plotF{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.60}{0.5cm}{-135}{$\eta_f$};
\plotE{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.25}{0.5cm}{   0}{$\xi$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 20.00
}
\plotRE{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.2}{0.5cm}{-90}{$R/\xi$};
\plotME{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.6}{0.5cm}{-45}{$M/\xi$};
\plotMRE{figures/propagating/data/rho0.20_p2_sts/data.txt} \plotpin{0.9}{0.5cm}{45}{$\eta/\xi$};
\end{plotpage}
\subcaption{$p=3$, $\tau^3 \sim h^2$}
}

\caption{Propagating wave example with $\rho=0.20$}
\label{figure_propagating_short}
\end{figure}

\subsubsection{Long-time error control}

We then consider $\rho=0.01$. We asymptotically obtain guaranteed bound
with effectitivity indices about $10$, except for $p=1$ where the asymptotic
regime is not really reached.

\begin{figure}
{
\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.4}{1cm}{10}{$\xi$};
\plotR{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.65}{0.5cm}{-45}{$R$};
\plotM{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.2}{0.5cm}{0}{$M$};
\plotF{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 300.00
}
\plotMRE{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.5}{0.5cm}{0}{$\eta/\xi$};
\plotRE{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-70}{$R/\xi$};
\plotME{figures/propagating/data/rho0.01_p0_r0.9/data.txt} \plotpin{0.35}{0.5cm}{-110}{$M/\xi$};
\end{plotpage}
\subcaption{$p=1$}

\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\plotR{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.55}{1cm}{-45}{$R$};
\plotM{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.3}{0.5cm}{0}{$M$};
\plotF{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 300.00
}
\plotMRE{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.5}{0.5cm}{ 20}{$\eta/\xi$};
\plotRE{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.8}{0.5cm}{ 90}{$R/\xi$};
\plotME{figures/propagating/data/rho0.01_p1_r0.9/data.txt} \plotpin{0.3}{0.5cm}{-90}{$M/\xi$};
\end{plotpage}
\subcaption{$p=2$}

\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\plotR{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.70}{1cm}{-45}{$R$};
\plotM{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.4}{0.5cm}{  0}{$M$};
\plotF{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 300.00
}
\plotMRE{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{ 10}{$\eta/\xi$};
\plotRE{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.95}{0.5cm}{ 90}{$R/\xi$};
\plotME{figures/propagating/data/rho0.01_p2_r0.9/data.txt} \plotpin{0.6}{0.5cm}{-90}{$M/\xi$};
\end{plotpage}
\subcaption{$p=3$}

\begin{plotpage}
{
	ymin = 1.e-6,
	ymax = 1.e+3
}
\plotE{figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.55}{1cm}{0}{$\xi$};
\plotR{figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.70}{1cm}{-45}{$R$};
\plotM{figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.4}{0.5cm}{  0}{$M$};
\plotF{figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.6}{0.5cm}{-135}{$\eta_f$};
\end{plotpage}
\begin{plotpage}
{
	ymin =   0.02,
	ymax = 300.00
}
\plotMRE{figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.60}{0.5cm}{ 90}{$\eta/\xi$};
\plotRE {figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.95}{0.5cm}{-90}{$R/\xi$};
\plotME {figures/propagating/data/rho0.01_p2_sts/data.txt} \plotpin{0.60}{0.5cm}{  0}{$M/\xi$};
\end{plotpage}
\subcaption{$p=3$, $\tau^3 \sim h^2$}
}

\caption{Propagating wave example with $\rho=0.01$}
\label{figure_propagating_long}
\end{figure}

\subsection{Time-step variation}

We finally investigate reducing the time-step for fixed meshes
for $p=2$ and $3$. To do so, for quadratic elements, with fix
$\tau$ using the CFL condition with $r=0.9,0.8,0.5,0.2$ and $0.1$.
For cubic elements, we select $\tau^3 \sim h^2$ as described above
with $r_0=0.9,0.8,0.5,0.2$ and $0.1$.
As can be seen on Figure \ref{figure_time_step}, reducing the
time-step has little effect on the actual error itself. However,
it does improve the efficiency of the estimator. In particular,
we obtain asymptotically-constant free bounds where $\tau$ is
selected ten times smaller than the CFL constraint. This is again
in agreement with the results in \cite{Theo:22} for the semi-discrete case.

\begin{figure}
{
\begin{plotpage}
{
	ymin=1.e-4,
	ymax=20,
	ylabel=$\xi$
}
\plotCFLE{figures/propagating/data/rho0.05_p1/data_0.800.txt}{thin,mark=square};
\plotCFLE{figures/propagating/data/rho0.05_p1/data_0.500.txt}{thin,mark=square};
\plotCFLE{figures/propagating/data/rho0.05_p1/data_0.200.txt}{thin,mark=square};
\plotCFLE{figures/propagating/data/rho0.05_p1/data_0.900.txt}{thick,mark=*}
\plotpin{0.7}{0.5cm}{ 45}{$r = 0.9$};
\plotCFLE{figures/propagating/data/rho0.05_p1/data_0.100.txt}{thick,mark=*}
\plotpin{0.9}{0.5cm}{180}{$r = 0.1$};
\end{plotpage}
\begin{plotpage}
{
	ymin=0.1,
	ymax=50,
	ylabel=$\eta/\xi$
}
\plotCFLMRE{figures/propagating/data/rho0.05_p1/data_0.800.txt}{thin,mark=square};
\plotCFLMRE{figures/propagating/data/rho0.05_p1/data_0.500.txt}{thin,mark=square};
\plotCFLMRE{figures/propagating/data/rho0.05_p1/data_0.200.txt}{thin,mark=square};
\plotCFLMRE{figures/propagating/data/rho0.05_p1/data_0.900.txt}{thick,mark=*}
\plotpin{0.3}{0.5cm}{  0}{$r = 0.9$};
\plotCFLMRE{figures/propagating/data/rho0.05_p1/data_0.100.txt}{thick,mark=*}
\plotpin{0.8}{0.5cm}{-45}{$r = 0.1$};
\end{plotpage}
\subcaption{$p=2$}

\begin{plotpage}
{
	ymin=1.e-4,
	ymax=20,
	ylabel=$\xi$
}
\plotCFLE{figures/propagating/data/rho0.05_p2/data_0.800.txt}{thin,mark=square};
\plotCFLE{figures/propagating/data/rho0.05_p2/data_0.500.txt}{thin,mark=square};
\plotCFLE{figures/propagating/data/rho0.05_p2/data_0.200.txt}{thin,mark=square};
\plotCFLE{figures/propagating/data/rho0.05_p2/data_0.900.txt}{thick,mark=*}
\plotpin{0.7}{0.5cm}{ 45}{$r_0 = 0.9$};
\plotCFLE{figures/propagating/data/rho0.05_p2/data_0.100.txt}{thick,mark=*}
\plotpin{0.9}{0.5cm}{180}{$r_0 = 0.1$};
\end{plotpage}
\begin{plotpage}
{
	ymin=0.1,
	ymax=50,
	ylabel=$\eta/\xi$
}
\plotCFLMRE{figures/propagating/data/rho0.05_p2/data_0.800.txt}{thin,mark=square};
\plotCFLMRE{figures/propagating/data/rho0.05_p2/data_0.500.txt}{thin,mark=square};
\plotCFLMRE{figures/propagating/data/rho0.05_p2/data_0.200.txt}{thin,mark=square};
\plotCFLMRE{figures/propagating/data/rho0.05_p2/data_0.900.txt}{thick,mark=*}
\plotpin{0.2}{0.5cm}{45}{$r_0 = 0.9$};
\plotCFLMRE{figures/propagating/data/rho0.05_p2/data_0.100.txt}{thick,mark=*}
\plotpin{0.9}{0.5cm}{-45}{$r_0 = 0.1$};
\end{plotpage}
\subcaption{$p=3$, $\tau^3 \sim h^2$}
}

\caption{Time step variation in the propagating wave example, $\rho=0.05$}
\label{figure_time_step}
\end{figure}

